Towards Flexible Inference in Sequential Decision Problems via Bidirectional Transformers

Randomly masking and predicting word tokens has been a successful approach in pre-training language models for a variety of downstream tasks. In this work, we observe that the same idea also applies naturally to sequential decision making, where many well-studied tasks like behavior cloning, offline RL, inverse dynamics, and waypoint conditioning correspond to different sequence maskings over a sequence of states, actions, and returns. We introduce the FlexiBiT framework, which provides a unified way to specify models which can be trained on many different sequential decision making tasks. We show that a single FlexiBiT model is simultaneously capable of carrying out many tasks with performance similar to or better than specialized models. Additionally, we show that performance can be further improved by fine-tuning our general model on specific tasks of interest.

==> sections/11-intro-old-notes.tex <==
% \MicahComment{Options for the introduction: 1) bringing bidirectionality and random masking from NLP to sequential decision processes; 2) proposing foundation models for sequential decision problems; 3) building on top of DT-type work; 4) multi-task literature, training on so many tasks that you learn to generalize to unseen ones}

% \MicahComment{One possible way to merge all three is: A perspective that has gaining traction is that of foundation models. In particular, in NLP has seen success with BERT. We build on top of specialized models for sequential decision problems such as DT, incorporating some of the insights of NLP to propose \fb{}.}

% \MicahComment{I don't really like foundation models \url{https://twitter.com/mer__edith/status/1429832405091856397}, but in a way there's no way to escape that}

%Recently there has been work on modeling sequential decision problems with transformers \citep{chen_decision_2021, janner_reinforcement_2021}. They use a decoder architecture (GPT) because of the forward-in-time character of most of their tasks but we can also use bi-directional models such as BERT, when used with appropriate masking. We show how that unlocks various additional modalities of inference that might be of interest, and enables to train a single model which is able to perform many different inference tasks, 
% Goal-conditioned behavior generation is enabled.
% Generation because it can be used both to do "RL" and IL.


Recent Success of DT - No need to constrain sequential decision models in the same way as NLP. What are the opportunities in sequential decision modelling when considering bidirectional models?

why limit ourselves to uni-directional? by using bi-directional, 1) train time, 2) test-time, and also enables us to explore potential for large models like in NLP


Masked Language Modeling \citep{devlin2018bert}, can apply to RL and sequential decision-making problems more broadly. Modeling bidirectional context has proven to be an important component of rich representations in NLP, where intuitively both the left and right context are useful for building the representation of a text token. In this work, we apply bidirectional transformers and masking schemes to sequential decision problems, leading to the surprising conclusion that in this context, masking is arguably more powerful than in language: while in language, masking was just an expedient for obtaining good representations (the applications we are interested in are not ``filling in the blanks'' with BERT), in sequential decision problems every masking scheme can have value in its own right as a meaningful task.

==> sections/50-complex-tasks.tex <==
\section{Mujoco experiments}
\label{sec:complex-envs}

Next, we report results for preliminary experiments on the HalfCheetah, Hopper, and Walker Mujoco environments~\citep{todorov2012mujoco}. We use the D4RL \emph{Mujoco medium expert datasets} \citep{fu2020d4rl} which we downsample to speed up experimentation.
%(Reacher didn't have a publicly available dataset)
%We report partial results below.% tasks as \citet{chen_decision_2021}
% , showing that our model is able to outperform DT, when both are used as behavior cloning models. However, we would like to 
%However, we preface these results with a word of skepticism about these environments, which, to us, seem inadequate for testing the generalization of learning algorithms. %These concerns ultimately led us to perform our full experiments on Maze2D, as we describe later.

% \prg{Limitations of benchmark environments.} We found that in the Mujoco tasks, using a single trajectory of data for training behavior cloning was sufficient to obtain relatively good performance (1000 vs. 1270 of the training trajectory on hopper), which increases even as the model dramatically overfits (as evidenced by the training loss being almost 0, and skyrocketing validation loss). Digging into the issue, it seemed that most of the problem arises from the fact that Mujoco's dynamics are deterministic: although there is some amount of randomness in the starting position, it doesn't seem to be sufficient for enough distributional drift to compound throughout a trajectory. That is, perfectly memorizing and regurgitating the training trajectory is sufficient to perform the task quite well. We believe this memorization property to be problematic, as it signifies that what is being tested is capacity for memorization rather than generalization. Moreover, the dataset used was obtained by a Markovian agent, leading the dataset to be fully Markovian, meaning that applying sequence models seems to be unnecessary. Nonetheless, for completeness we report here our preliminary results. % (obtained before we realized the extent of the problems with the environments).
% \sm{small thing, but there's a lot of tense disagreement throughout. for example, when presenting the results, many of the statements are in present tense. however, the limitations of the benchmark environment section is written in past tense. recommend a bit more tense agreement.}


% We test our method also in the more complex environments used by \citet{chen_decision_2021}, Mujoco and Atari. 
% While the size of the Atari dataset is a bottleneck for performance (we found that even reducing the size of the data by $10\%$ visibly affected performance),

%\prg{Dataset.} 
%For our tasks, we use the D4RL Mujoco ``medium'' datasets \cite{} which we downsample for speeding up experimentation time. %and 2) obtaining larger effect sizes between models (even drastically reducing the amount of data (e.g., by $95\%$) leads to almost unaffected performance for Behavior Cloning). %We initially found that even drastically reducing the amount of data (e.g., by $95\%$) leads to almost unaffected performance for Behavior Cloning. 
%For rendering the Mujoco domain data-bottlenecked, we downsample their datasets until performance starts being affected, as described in \secref{}.
% \sm{this section is a little confusing to a reader. 1) what do you mean by "initially found"? 2) how does that influence the next part about the mujoco datasets? 3) what procedure do you actually do to sample all of the datasets? we don't need to necessarily communicate the things we tried.}

\prg{Task setup.} We evaluate models exclusively on the behavior cloning task, considering cumulative reward in evaluation rollouts as the performance metric (unlike in the minigrid experiments). We again compare the performance of \fb when using several training regimes introduced in \Cref{sec:masking_schemes}, namely, \bcmask, \rndmask, and \ftmask. Additionally, we baseline with a simple Neural Network model trained to perform behavior cloning (NN-BC), and with a Decision Transformer \citep{chen_decision_2021} trained without rewards-to-go\footnote{This is equivalent to using a GPT-like model to perform behavior cloning---used in the original paper for their Atari BC baselining.} (\DTBC). %For \fb, we experimented with three different regimes: 1) \bcmask masking, which implements behavior cloning as in \Cref{subsec:masking_schemes}; 2) \rndmask masks, which uses a uniformly random masking during training time; and 3) \ftmask, which is finetunes an \rndmask-trained model on \bcmask masking.
See \cref{sec:mujoco-details} for more details about the setup.

 %First, as a sanity check, we see that DT-BC and \fb{} with last\_action masking perform similarly across all domains. This is to be expected since, with this masking, the two networks and their training are almost identical; the only difference is that DT-BC uses a GPT architecture while \fb{} uses a BERT one. \fb{} performs slightly worse on 2/3 domains, which is expected considering the downsides of using BERT for sequence generation \cite{} \orrp{Cite here? BERT paper?}, plus a minor mis-match in the masking that puts last\_action at a disadvantage (see \Cref{tmp} \orrp{ref here once it exists}).   

\prg{Results.} Across all environments considered, the best reward is obtained by first training a \fb model with random masking and then fine-tuning it to the BC task. This further supports \textbf{H1} and \textbf{H4}. Among the specialized models, \fb performs surprisingly well, generally outperforming its GPT-based and NN-based counterparts. \fb trained on RND alone lags behind in performance relative to the specialized BC model, but performs similarly to NN-BC and DT-BC (partially supporting \textbf{H2}).

% \prg{Increasing randomization.} We see that depending on the domain, increasing randomization seems to be able to directly increase the reward. 

% \prg{Why do neural networks perform so well?} Looking at the NN column of \tableref{}, we see that a simple neural network trained to perform last action prediction does surprisingly well. While this warrants further investigation, we believe this is in part due to Mujoco's and D4RL's idiosyncrasies: in particular the way that all D4RL datasets were created -- rolling out neural-network agents \MicahComment{double check, was it fed multiple states?}, potentially leading this model form choice to provide a better inductive bias in low-data regimes than using a transformer network. See \Appref{} \MicahComment{Would be nice to add an experiment with a Transformer-A2C policy and verify that this doesn't still happen -- could also have to do with model size/num of params}. For example, we don't see this happening in the Atari domain \MicahComment{verify this. Was atari data also created with a neural network?}. This is also specific to the low-data regime: once in high data regime, the NN and transformers obtain similar performance. To us, this simply is a testament to the fact that simple neural networks are better at memorization in this environments, due to the problems mentioned previously -- and motivated our transition to Maze2D. 

% \begin{figure}[h]
%   %\vskip 0.2in
%   \centering
%   \includegraphics[width=\linewidth]{images/mujoco_results.png}
%   \caption{\textbf{Mujoco comparison with DT.}}\vspace{-1em}
%   \label{fig:example}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\begin{tabular}{@{}llllll@{}}
\toprule
\textbf{Environment} & \bNN & \bDTBC & \bfb\textbf{-}\bbc & \bfb\textbf{-}\brnd & \bfb\textbf{-}\bft \\ \midrule
Hopper      & $1579\mypm 290$        & $1472\mypm 162$          & $1534\mypm 100$                           & $1413\mypm 215$                            & $\mathbf{1610\mypm 63}$                            \\
HalfCheetah & $3616\mypm 181$        & $3781\mypm 178$          & $4286\mypm 131$                           & $3451\mypm 435$                            & $\mathbf{4466\mypm 117}$                           \\
Walker      & $2487\mypm 234$        & $2626\mypm 158$          & $2811\mypm 170$                           & $2565\mypm 125$                            & $\mathbf{2969\mypm 113}$                           \\ \bottomrule
\end{tabular}
\caption{We see that across the various Mujoco environments, the best reward is obtained by training a \fb model with random masking and then fine-tuning it to BC. We report the standard errors over reward evaluations performed by 3 different models (with different seeds).}\label{table:mujoco}
\end{table}

% \subsection{Maze2D Environment}

% % We initially set out to compare the performance of \fb{} on the same continuous control tasks used in \citet{chen_decision_2021}. However, noticing that completely overfitting a single trajectory with a multi-layer perceptron was sufficient to obtain good reward performance, we concluded that such environments don't have enough inherent randomness to be a good indicator as to the generalization of the trained policies -- which is what we ultimately care about. \MicahComment{markovian policy} More about these experiments is reported in \Appref{}. 



% \prg{Maze2D Environment.} We choose a continuous control environment that is not plagued by the issues above: a custom version of Maze2D~\cite{fu2020d4rl}. In this environment, a point-mass object is placed at a random location in a maze, and is rewarded for reaching a random target location. Memorizing a single trajectory in this setup leads to poor performance, as the initial position and goal location at evaluation time will almost certainly be different. The timestep-reward is the percentage of distance covered between the initial position and the target position -- this has the advantage of leading to interpretable cumulative rewards: $70$ means that the agent was able to get $70\%$ of the way towards the goal. We additionally make the task harder by: 1) increasing the amount of initial position randomization and 2) remove velocity from each timestep's observation. This forces models trained on this data to have to implicitly infer the agent's velocity from observed context.

% \prg{Dataset generation.} We generate our data using D4RL's PD controller with a bug fixed. \MicahComment{move mention of the bug to the appendix, with description of it} The fact that such PD controller is non-Markovian is another advantage over using DT's environments: the datasets for their continuous control task were generated with agents parametrized with simple feed-forward networks, meaning that a sequence model is unnecessary to capture their behavior. \MicahComment{check} We generate 35 trajectories of 200 timesteps each, 30 of which are used for validation, and 5 for training -- given the simplicity of the task. The average reward in the training data is $97$, meaning that within this horizon, the PD controller is almost always able to reach the target location perfectly.

% % (1000 timesteps for training and)%To increase the randomness of the environment, and make the task harder, we generated a new dataset rather than using the ones provided out-of-the-box by D4RL: we still use D4RL's non-Markovian PD controller (but fixing a bug in it's code);  By removing velocity from the 

% % We use D4RL's non-Markovian PD controller. We did not use D4RL's dataset, as we found a bug in \citep{d4rl}'s dataset generation process, and the task was too easy to see any meaningful differences between models. We 

% %  -- with a bug fixed. To make the Maze2D task more challenging, we also perform some changes to : the starting location % collection of datasets -- which have varying performances for each environment. We focus on the "medium" dataset -- obtained by rolling out a partially trained RL policy. %Given that we are interested in investigating the data-augmentation effect of our masking scheme on tasks which include Behavior Cloning, we reduced the amount of data until performance started being affected significantly: for training we only consider a randomly-selected subset of the "medium" dataset which has $0.5\%$ of the original number of trajectories.

% \prg{Models trained.} We train \fb{} models with different masking randomization schemes, as done in \secref{}, and evaluate each model on two downstream tasks: behavior cloning and DT-style offline-RL (reward-conditioned behavior cloning). We compare these models with DT.



% \MicahComment{using neural network rather than transformer with maskings}
% \MicahComment{ablation on stacking}
% \MicahComment{ablation on first-reward}

% \MicahComment{try larger seq len}
% \MicahComment{try larger maze env}
% \MicahComment{try more data}
% \MicahComment{do more hyperparam tuning}
% \MicahComment{re-run medium with split which has worse average performance?}
% \MicahComment{try fine-tuning}



% \prg{Behavior Cloning results.} As a first sanity check, note that \fb{}, when trained to simply predict the last action performs comparably to DT. As


% \prg{Reward-conditioned setup.}

% \prg{Reward-conditioned results.}

% \prg{Waypointing setup.}

% \prg{Waypointing results.}

% \MicahComment{mention different way of handling rewards-to-go}



% \begin{table*}[t]
% \centering
% \small
% \begin{tabular}{lcccccc}\toprule
% & \multicolumn{3}{c}{\textsc{BC}} & \multicolumn{3}{c}{\textsc{Dataset}} \\ 
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}
% \bf Model & Hopper & Rec. & F$_{0.5}$ & Prec. & Rec. & F$_{0.5}$ \\\midrule
% MT      & 3.3 & \bf 31.4 & 4.0   & 16.2 & \bf 78.6 & 19.2      \\
% GEC     & 52.8 & 6.6 & 22.0    & 78.0 & 53.3 & 71.4       \\
% APE     & 51.2 & 7.3 & 23.3    & 78.1 & 54.4 & 71.8     \\
% BERT-APE & 6.8 & 10.8 & 7.3     & 32.0 & 57.8 & 35.1  \\
% \midrule
% \textsc{Model} & \bf 57.4 & 9.4 & \bf 28.4  & \bf 82.1 & 57.2 & \bf 75.5 \\
% \bottomrule
% \end{tabular}
% \caption{}
% \label{tab:results}
% \end{table*}




% \begin{minipage}[c]{\textwidth}

% \setlength\tabcolsep{1.5pt}
% \begin{tabular}[b]{cccccc}
%     &  & \multicolumn{4}{c}{\textbf{Oracle Training}} \\
%     \cmidrule(lr){3-6}
%     & & \multicolumn{2}{c}{\textit{Unpenalized}} & \multicolumn{2}{c}{\textit{Penalized}} \\
%     % \cmidrule(lr){3-4}\cmidrule(lr){5-6}
%     & & Myopic & RL & Myopic & RL \\
%     \cline{2-6}
%     \parbox[t]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Oracle Eval}}}}
%     & $\rew_t(\pref_t^{\pi'})$ & 5.71 & 7.49  & 6.20 & 5.28 \\
%     & $\rew_t(\pref_0, \pi')$ & 1.99 & -0.08 & 3.61 & 6.21 \\
%     & $\rew_t(\pref_t^{\pi_{\text{rnd}}}, \pi')$ & 2.01 & -1.09 & 3.10 & 4.57 \\
%     & Sum      & 9.69 & 6.33  & 12.90 & 16.05 \\
%     \cline{2-6}
% \end{tabular}
% \captionof{table}{}
% \label{table:results1}
% \end{minipage}\quad
% \begin{minipage}[c]{\textwidth}
% \setlength\tabcolsep{1.5pt}
% \begin{tabular}[b]{cccccc}
% &  & \multicolumn{2}{c}{\textbf{Oracle Training}} & \multicolumn{2}{c}{\textbf{Training in Sim.}} \\
% \cmidrule(lr){3-4}\cmidrule(lr){5-6}
% & & \textit{Unpen.} & \textit{Penal.} & \textit{Unpen.} & \textit{Penal.} \\
% \cline{2-6}
% \parbox[t]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Oracle Eval}}}}
% & $\rew_t(\pref_t^{\pi'})$ &  7.49 & 5.28 &  6.40 & 5.48 \\
% & $\rew_t(\pref_0, \pi')$ & -0.08 & 6.21 & -1.24 & 5.61 \\
% & $\rew_t(\pref_t^{\pi_{\text{rnd}}}, \pi')$ & -1.09 & 4.57 & -1.83 & 4.43 \\
% & Sum      &  6.33 & 16.05 &  3.36 & 15.52 \\
% \cline{2-6}
% \parbox[t]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Est. Eval}}}}
% & $\rew_t(\pref_t^{\pi'})$ & 5.58 & 5.42  & 6.49 & 5.78 \\
% & $\rew_t(\pref_0, \pi')$ & 1.28 & 5.57  & -0.80 & 4.94 \\
% & $\rew_t(\pref_t^{\pi_{\text{rnd}}}, \pi')$ & 2.05 & 3.88  & 1.48 & 4.41 \\
% & Sum      & 8.91 & 14.87  & 7.17 & 15.15 \\
% \cline{2-6} 
% \end{tabular}
% \label{table:resultsHMEST}
% \captionof{table}{}
% \vspace{-1em}
% \end{minipage}

% \subsection{Atari}

% \prg{Data.}

% \prg{Behavior Cloning setup.} 

% \prg{Behavior Cloning results.}

% \prg{Reward-Conditioned setup.}

% \prg{Reward-Conditioned results.}

% \begin{figure*}[h]
%   %\vskip 0.2in
%   \centering
%   \includegraphics[width=\textwidth]{images/atari_results.png}
%   \caption{\textbf{Atari comparison with DT.} TODO}\vspace{-1em}
%   \label{fig:example}
% \end{figure*}

% \subsection{Bleeding Edge}

% Bleeding Edge is modern 4v4 online video game. We compared the performance of \fb{} with DT-BC on human-generated gameplay sessions.

% \prg{Data.} The data used for training

% \prg{Behavior Cloning setup.} 

% \prg{Behavior Cloning results.}
